Bounds for tentacular Hamiltonians

This paper represents a first step towards the extension of the definition of Rabinowitz Floer homology to non-compact energy hypersurfaces in exact symplectic manifolds. More concretely, we study under which conditions it is possible to establish $L^{\infty}$-bounds for the Floer trajectories of a Hamiltonian with non-compact energy levels. Moreover, we introduce a class of Hamiltonians, called tentacular Hamiltonians, which satisfy the conditions: how to define RFH for these examples will be the subject of a follow-up paper.

==> abstract.tex <==
\markboth{F. Pasquotto and J. Wi\'{s}niewska}{Bounds for tentacular Hamiltonians}



\title{BOUNDS FOR TENTACULAR HAMILTONIANS}

\author{FEDERICA PASQUOTTO}

\address{Department of Mathematics, Vrije Universiteit Amsterdam,\\
De Boelelaan 1081, 1081 HV Amsterdam, Netherlands\\
f.pasquotto@vu.nl}

\author{JAGNA WI\'{S}NIEWSKA}

\address{Department of Mathematics, ETH Z\"{u}rich, \\
Raemistrasse 101, 8092 Z\"{u}rich, Switzerland \\
jagna.wisniewska@math.ethz.ch}

\maketitle


\begin{abstract}
This paper represents a first step towards the extension of the definition of Rabinowitz Floer homology to non-compact energy hypersurfaces in exact symplectic manifolds. More concretely, we study under which conditions it is possible to establish $L^\infty$-bounds for the Floer trajectories of a Hamiltonian with non-compact energy levels. Moreover, we introduce a class of Hamiltonians, called \textit{tentacular Hamiltonians} which satisfy the conditions: how to define RFH for these examples will be the subject of a follow-up paper. 
\end{abstract}

\keywords{Rabinowitz Floer Homology, non-compact hypersurfaces, Morse-Bott action functional, Alexandrov's maximum principle}


\ccode{AMS Subject Classification: 53D40, 57R17, 58J05}
